On the Effectiveness of Adapter-based Tuning for Pretrained Language Model Adaptation

Adapter-based tuning has recently arisen as an alternative to fine-tuning. It works by adding light-weight adapter modules to a pretrained language model (PrLM) and only updating the parameters of adapter modules when learning on a downstream task. As such, it adds only a few trainable parameters per new task, allowing a high degree of parameter sharing. Prior studies have shown that adapter-based tuning often achieves comparable results to fine-tuning. However, existing work only focuses on the parameter-efficient aspect of adapter-based tuning while lacking further investigation on its effectiveness. In this paper, we study the latter. We first show that adapter-based tuning better mitigates forgetting issues than fine-tuning since it yields representations with less deviation from those generated by the initial PrLM. We then empirically compare the two tuning methods on several downstream NLP tasks and settings. We demonstrate that 1) adapter-based tuning outperforms fine-tuning on low-resource and cross-lingual tasks; 2) it is more robust to overfitting and less sensitive to changes in learning rates.

==> acl-ijcnlp2021-templates/tables/table_ner_main_comparison.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Model & \bf{All} & \bf{Target} & \bf{Distant} \\
\midrule
XLMR-ft \citep{hu2020b} & 65.40 & 64.87 & 58.21 \\
XLMR-ft (reproduced) & 63.85 & 63.32 & 56.85 \\
\midrule
XLMR-adapter$_{128}$ & 63.41 & 62.93 & 55.84 \\
XLMR-adapter$_{256}$ & \textbf{66.40} & \textbf{65.95} & \textbf{59.01} \\
XLMR-adapter$_{384}$ & 66.08 & 65.62 & 58.87 \\
\bottomrule
\end{tabular}}
\caption{Zero-shot cross-lingual NER F1. \textbf{All} is the average test F1 of all languages. \textbf{Target} is the average test F1 of all target languages expect English. \textbf{Distant} is the average test F1 of the languages not in the Indo-European family.}
\label{table:ner_main_comp}
\end{table}

==> acl-ijcnlp2021-templates/tables/table_pos_main_comparison.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Model & \bf{All} & \bf{Target} & \bf{Distant} \\
\midrule
XLMR-ft \citep{hu2020b} & 73.80 & 73.14 & 64.34 \\
XLMR-ft (reproduced) & 74.29 & 73.61 & 64.90 \\
\midrule
XLMR-adapter$_{64}$ & 74.81 & 74.15 & 66.13 \\
XLMR-adapter$_{256}$ & 75.82 & 75.20 & \textbf{68.05}\\
XLMR-adapter$_{384}$ & 75.56 & 74.92 & 66.91\\
XLMR-adapter$_{512}$ & \textbf{76.01} & \textbf{75.38} & 67.81 \\
\bottomrule
\end{tabular}}
\caption{Zero-shot cross-lingual POS tagging accuracy. \textbf{All} is the average test accuracy of all languages. \textbf{Target} is the average test accuracy of all target languages expect English. \textbf{Distant} is the average test accuracy of the languages not in the Indo-European family.}
\label{table:pos_main_comp}
\end{table}

==> acl-ijcnlp2021-templates/tables/table_xnli_high.tex <==
\begin{table}[!]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Model & \bf{All} & \bf{Target} & \bf{Distant} \\
\midrule
XLMR-ft \citep{hu2020b} & 79.24 & 78.56 & 76.73 \\
\midrule
XLMR-adapter$_{64}$ & 79.59 & 79.01 & 77.18 \\
XLMR-adapter$_{128}$ & 79.83 & 79.24 & 77.40 \\
XLMR-adapter$_{256}$ & \textbf{80.08} & \textbf{79.43} & \textbf{77.60} \\
XLMR-adapter$_{384}$ & 79.10 & 78.41 & 76.60 \\
\bottomrule
\end{tabular}}
\caption{Zero-shot XNLI accuracy for the high-resource setting.}
\label{table:xnli_high_resource}
\end{table}
